Learning to Cut by Watching Movies

Video content creation keeps growing at an incredible pace; yet, creating engaging stories remains challenging and requires non-trivial video editing expertise. Many video editing components are astonishingly hard to automate primarily due to the lack of raw video materials. This paper focuses on a new task for computational video editing, namely the task of raking cut plausibility. Our key idea is to leverage content that has already been edited to learn fine-grained audiovisual patterns that trigger cuts. To do this, we first collected a data source of more than 10K videos, from which we extract more than 255K cuts. We devise a model that learns to discriminate between real and artificial cuts via contrastive learning. We set up a new task and a set of baselines to benchmark video cut generation. We observe that our proposed model outperforms the baselines by large margins. To demonstrate our model in real-world applications, we conduct human studies in a collection of unedited videos. The results show that our model does a better job at cutting than random and alternative baselines.

==> figures/lenght_distribution.tex <==
\begin{figure}[t!]
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/shots_durations_hist.pdf} 
  \caption{\textbf{Distribution of shot lengths in MovieCuts} We observe a strong bias in MovieCuts towards short clips, this distribution emphasizes the importantce of automatic tools to support the edition process as most editors prefer to align multiple short short instead of few long sequences.}
\label{fig:shots-duration}
\end{figure}

==> figures/multistage_params.tex <==
\begin{figure}[h!]
    \begin{center}
        \includegraphics[width=0.95\columnwidth]{images/top_k_plot.pdf}
    \end{center}
    \caption{\textbf{Multi-stage inference: influence of $M$.} We present the influence of $M$ for our model using different streams. We compare this values using only $R@1K$ Purple shows our model using only the visual stream, pink only audio, and yellow video-audio.}
    \label{fig:multistage}
\end{figure}

==> figures/statistics.tex <==
\begin{figure}[t!]
  \centering
         \centering
         \includegraphics[width=\linewidth]{images/statistics.pdf} 
        \label{fig:shots-duration}
        \caption{\textbf{Dataset Statistics}. Figure a shows the distribution per genre. The dataset contain scenes from more than 20 movie categories. The two larger genres are Comedy and Drama, followed by Action, Crime, and Adventure. ``Others" category includes Documentaries, Film-Noir, Musicals, News, Short movies, War, and Western. Figure b shows the duration distribution. We observe a strong bias towards short clips, this distribution emphasizes the importance of automatic tools to support the edition process as most editors prefer to align multiple short short instead of few long sequences.}
        \label{fig:statistics}
\end{figure}


==> tables/ablation.tex <==
% \begin{table}[t]
% \footnotesize
% \setlength{\tabcolsep}{5pt}
% \centering\footnotesize
% \begin{tabular}{lcc}
% \toprule
% Method                         & R$@1K$($d=1$)         & R$@1K$($d=2$)   & R$@1K$($d=2$) \\ \midrule
% \textsc{\textbf{Ours}}          & $31.57$                 & $0.00$     & $0.00$      \\ \midrule
% % Ours (\textit{w/o multi-stage}) & $0.00$                 & $0.00$     \\ \midrule
% w/o auxiliary task              & $17.47$                 & $0.00$     & $0.00$      \\
% w/o audio                       & $14.90$                 & $0.00$      & $0.00$     \\
% w/o visual                      & $9.26$                 & $0.00$      & $0.00$     \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Ablation study.}}
% \label{table:ablation}
% \end{table}

\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{0.8pt}
\begin{tabular}{@{}c@{\hspace{0.4em}} l c@{\hspace{0.2em}} cc c@{\hspace{0.2em}} cc c@{\hspace{0.2em}} cc c@{\hspace{0.2em}} c@{}}
\toprule
&& \phantom{} & \multicolumn{2}{c}{$d=1$} &  \phantom{} & \multicolumn{2}{c}{$d=2$} &  \phantom{} & \multicolumn{2}{c}{$d=3$} & \phantom{} \\
\cmidrule{3-5} \cmidrule{7-8} \cmidrule{10-12} 
& Model && R$@1K$ & R$@5K$ && R$@1K$ & R$@5K$  && R$@1K$ & R$@5K$  \\
\midrule
&\textbf{LTC (Full)} && 8.18 & 24.44 && 15.30 & 48.26  && 19.18 & 64.30 \\
\midrule
% &w/o visual && 7.82 & 24.65 && 14.99 & 48.21  && 18.96 & 64.07 \\
&w/o audio && 6.30 & 22.65 && 12.61 & 44.56  && 16.54 & 59.37 \\
&w/o auxiliary  && 4.91 & 20.64  && 10.08 & 43.95 && 13.78 & 61.29 \\

\bottomrule
\end{tabular}
\caption{\textbf{Ablation study.}  We evaluate our method against its variants: without the visual stream, without the audio stream, and without the auxiliary task. We report only $R@1K$ and $R@5K$ for ease of comparison.} 
\label{table:ablation}
\end{table}


==> tables/generalization.tex <==
\begin{table*}[!ht]
\footnotesize
\small
\begin{tabular}{@{}c@{\hspace{0.4em}} l c@{\hspace{0.2em}} ccc c@{\hspace{0.2em}} ccc c@{\hspace{0.2em}} ccc c@{\hspace{0.2em}} c@{}}
\toprule
&& \phantom{} & \multicolumn{3}{c}{$d=1$} &  \phantom{} & \multicolumn{3}{c}{$d=2$} &  \phantom{} & \multicolumn{3}{c}{$d=3$} & \phantom{} \\
\cmidrule{4-6} \cmidrule{8-10} \cmidrule{12-14} 
& Model && R$@1K$ & R$@5K$  & R$@10K$ && R$@1K$ & R$@5K$  & R$@10K$  && R$@1K$ & R$@5K$  & R$@10K$  \\
\midrule
&Random && 0.83 & 3.33 & 3.33 && 1.67 & 8.33 & 15.00 && 3.33 & 17.50 & 30.00\\
&Audio-visual && 1.67 & 4.17 & 5.00 && 2.50 & 5.83 & 10.83 && 2.50 & 11.67 & 20.00\\
&\textsc{\textbf{Ours}} && 0.83 & 2.50 & 8.33 && 1.67 & 10.83 & 30.83 && 5.83 & 17.50 & 34.67 \\
\bottomrule
\end{tabular}
\caption{\textbf{Generalization to unedited videos.} We showcase our model's results in a real-case scenario where it processes raw unedited footage. We report the same metrics as before by comparing our results with the cuts of professional editors.} 
\label{table:generalization}
\end{table*}


==> tables/humanstudy.tex <==
\begin{table}[!ht]
\footnotesize
% \setlength{\tabcolsep}{10pt}
\small
\tabcolsep=0.07cm

\begin{subtable}{\linewidth}
\centering

\caption{Absolute counts} \label{table:human-study-counts}
\begin{tabular}{l c c c c c}
\toprule
% & \multicolumn{4}{c}{Count} \\
% \cmidrule{2-5}
& Random & Audio-visual & Ours & Pros \\
\midrule
General audience & $43.4$ & \underline{$45.8$} & $43.7$ & $\mathbf{67.1}$ \\
Professional editors & $39.7$ & $41.4$ & \underline{$47.8$} & $\mathbf{71.1}$\\
\bottomrule
\end{tabular}
\end{subtable} \\

\begin{subtable}{\linewidth}
\centering
\vspace{5pt}
\caption{Percentage chosen over professional cuts} \label{table:human-study-pros}
\centering
\begin{tabular}{l c c c c}
\toprule
% &  \multicolumn{3}{c}{Compared to Pros} \\
% \cmidrule{2-4}
& Random & Audio-visual & Ours \\
\midrule
General audience &  $29.6$ & $\mathbf{36.2}$ & $33.0$ \\
Professional editors & $26.7$ & $27.5$ & $\mathbf{32.5}$ \\
\bottomrule
\end{tabular}
    
\end{subtable}
\caption{\textbf{Human study.} Table (a) shows the absolute number of times that the general audience (first row) and the professional editors (second row) preferred each source of cuts (Random, Audio-visual, Ours, Pros). Table (b) shows the percentage of times that general audience (first row) and professional editors (second row) preferred each source of cut over the professional cuts.}
\label{table:humanstudy}
\end{table}

